Efficient sampling from the Bingham distribution

We give a algorithm for exact sampling from the Bingham distribution $p(x)\propto \exp(x^\top A x)$ on the sphere $\mathcal S^{d-1}$ with expected runtime of $\operatorname{poly}(d, \lambda_{\max}(A)-\lambda_{\min}(A))$. The algorithm is based on rejection sampling, where the proposal distribution is a polynomial approximation of the pdf, and can be sampled from by explicitly evaluating integrals of polynomials over the sphere. Our algorithm gives exact samples, assuming exact computation of an inverse function of a polynomial. This is in contrast with Markov Chain Monte Carlo algorithms, which are not known to enjoy rapid mixing on this problem, and only give approximate samples. As a direct application, we use this to sample from the posterior distribution of a rank-1 matrix inference problem in polynomial time.

==> formatting.tex <==
\renewcommand{\thesection}{\arabic{section}}

==> lowerbound.tex <==
\section{Lower bound for rejection sampling with normalized Gaussian proposal}

In this section, we show that if we wish to do sampling with a normalized Gaussian, there are simple instances where the worst-case ratio with the desired distribution can be arbitrarily bad, even in dimension $d=2$. 

Define an \emph{angular Gaussian distribution} as any distribution over $\mathcal S^{d-1}$ in the form
 $p(x) =\frac{(x^T \Omega x)^{-d/2}}{\det(\Omega)^{1/2}}$. This is a normalized Gaussian distribution with covariance matrix $\Sigma$, where
 where $\Omega = \Sigma^{-1}$. %and $\Sigma$ is the covariance matrix of the Gaussian we are renormalizing. 
 
 We show the following, which shows that for the circle $\cal S^1$, the ratio between a Bingham distribution and \emph{any} angular Gaussian distribution can become arbitrarily large.
 \begin{lem} Let $q:\mathbb{R}^2 \to \mathbb{R}$ be defined as $q(x) = \frac{e^{x_1^2 \sigma^2}}{Z}$. Furthermore, for any positive-definite $\Omega \in \mathbb{R}^{2 \times 2}$, let  $p_{\Omega}(x) =\frac{(x^T \Omega x)^{-1}}{\det(\Omega)^{1/2}}$.
 
Then, as  
 $\sigma \to \infty$, 
$\min_{\Omega} \max_{x \in \mathcal{S}^d} \max \left\{\frac{p_{\Omega}(x)}{q(x)},{\frac{q(x)}{p_{\Omega}(x)}} \right\} \to \infty $.
 \end{lem} 
 \begin{proof}
 
Suppose otherwise for the sake of contradiction. First, we have 
\begin{align*}
    \frac{q((1,0))}{q((0,1))} = e^{\sigma^2}
\end{align*}
 so correspondingly, we need to have $\frac{p_{\Omega}((1,0))}{p_{\Omega}((0,1))} = \frac{\Omega^{-1}_{11}}{\Omega^{-1}_{22}} \to \infty$, i.e. $\frac{\Omega_{11}}{\Omega_{22}} \to 0$ 
 
 We also have 
 \begin{align*}
    \frac{q((1,0))}{q((1/2,1/2))} = e^{3/4 \sigma^2}
\end{align*}
and 
 \begin{align*}
    \frac{p_{\Omega}((1,0))}{p_{\Omega}((1/2,1/2))} = \frac{\Omega^{-1}_{11}}{4 (\Omega_{11}+\Omega_{22} + \Omega_{12})^{-1}}
\end{align*}
Since $\Omega$ is a positive definite matrix, we have $|\Omega_{12}| \leq \sqrt{\Omega_{11} \Omega_{22}}$, so in particular, \begin{align} \Omega_{11}+\Omega_{22} + \Omega_{12} &\geq \Omega_{22} - \Omega_{11} - \sqrt{\Omega_{22} \Omega_{11}}
\end{align} 
Note that $\frac{\sqrt{\Omega_{22}\Omega_{11}}}{\Omega_{22}} \to 0$, so that $\Omega_{22} - \Omega_{11} - \sqrt{\Omega_{22} \Omega_{11}} \to \Omega_{22}$. 

 But then, we have that 
 $\frac{q((0,1))}{q((1/2,1/2))} = e^{-1/4 \sigma^2} \to 0$, while $\frac{p_{\Omega}((0,1))}{p_{\Omega}((1/2,1/2))} \to 1/4$, which is a contradiction. 
 
 
 %Since $\sigma \to \infty$, it's clear that $\Omega$ has to be of the form where $\forall (i,j) \neq (1,1), \frac{\Omega_{11}^2}{\Omega{ij}^2} \to \infty$. 
 
 
 %Consider first $x$, s.t. $x_1 \to 0$. We have: 
 %\begin{align*}
%\log p_{\Omega}(x) \approx -\frac{1}{2} \log \mbox{det}(\Omega)-\frac{d}{2} \log\left(\sum_{(i,j)\neq(1,1)}\Omega_{i,j} x_i x_j\right)- \frac{\frac{d}{2} x_1^2}{\sum_{(i,j)\neq(1,1)}\Omega_{i,j} x_i x_j} \Omega^2_{11}  
% \end{align*}
% On the other hand, as $x_1 \to 1$, we have 
% \begin{align*}
%\log p_{\Omega}(x) \approx -\frac{d}{2} \log \Omega_{11}-\frac{1}{2} \log \mbox{det}(\Omega) 
%\end{align*}
 
 
 %Consider the same calculation for $\sigma$. For small enough $x_1$, we have $e^{x_1^2 \sigma^2} \approx 1 + x_1^2 \sigma^2$. Hence, for $x_1 \to 0$, we have
 %$$\log q(x) \approx x_1^2 \sigma^2 - \log Z $$
 %On the other hand, for $x_1 \to 1$, we have 
 %$$\log q(x) \approx e^{\sigma^2} - \log Z$$ 
 
 %Hence, as $\sigma \to \infty$, $p_{\Omega}(x) \to \frac{(x^2_1 \Omega^2_{11} + \sum_{\i \neq j} \Omega_{i,j} x_i x_j )^{-d/2}}{\mbox{det}(\Omega)}$.
 
 
 %For small enough $x_1$, we have $e^{x_1^2 \sigma^2} \leq 1 + 2 x_1^2 \sigma^2$. Hence, for small enough $x_1$, $q(x) \leq e^{x_1^2 \sigma^2}/Z$. 
 %On the other hand, for small enough $x_1$, 
 %$$p_{\Omega}(x) = $$
 

 
 
 \end{proof}

==> macros-alt.tex <==
%LETTERS

%UPPERCASE
\newcommand{\sA}[0]{\mathscr{A}}
\newcommand{\cA}[0]{\mathcal{A}}
\newcommand{\A}[0]{\mathbb{A}}
\newcommand{\cB}[0]{\mathcal{B}}
\newcommand{\C}[0]{\mathbb{C}}
\newcommand{\sC}[0]{\mathcal{C}}%deprecated
\newcommand{\cC}[0]{\mathcal{C}}
\newcommand{\sD}[0]{\mathscr{D}}
\newcommand{\mD}[0]{\mathfrak D}
\newcommand{\cE}[0]{\mathscr{E}}%deprecated
\newcommand{\sE}[0]{\mathscr{E}}
\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\EE}[0]{\mathop{\mathbb E}}
%\scalebox{1.25}{$\mathbb E$}}
\newcommand{\F}[0]{\mathbb{F}}
\newcommand{\cF}[0]{\mathcal{F}}
\newcommand{\sF}[0]{\mathscr{F}}
\newcommand{\G}[0]{\mathbb{G}}
\newcommand{\cG}[0]{\mathscr{G}}%deprecated.
\newcommand{\sG}[0]{\mathscr{G}}
\newcommand{\cH}[0]{\mathscr H}%deprecated
\newcommand{\sH}[0]{\mathscr H}
\newcommand{\Hq}[0]{\mathbb{H}}
\newcommand{\bfI}[0]{\mathbf{I}}
\newcommand{\I}[0]{\mathbb{I}}
\newcommand{\cI}[0]{\mathscr{I}}%deprecated
\newcommand{\sI}[0]{\mathscr{I}}
\newcommand{\cJ}[0]{\mathscr{J}}
\newcommand{\cK}[0]{\mathcal{K}}
\newcommand{\sL}[0]{\mathscr{L}}
\newcommand{\mM}[0]{\mathfrak{M}}
\newcommand{\N}[0]{\mathbb{N}}
\newcommand{\fN}[0]{\mathfrak{N}}
\newcommand{\cP}[0]{\mathcal{P}}
\newcommand{\Pj}[0]{\mathbb{P}}
\newcommand{\sP}[0]{\mathscr{P}}
\newcommand{\mP}[0]{\mathfrak{P}}
\newcommand{\mQ}[0]{\mathfrak{Q}}
%!
\newcommand{\cO}[0]{\mathcal{O}}
\newcommand{\sO}[0]{\mathscr{O}}
\newcommand{\Q}[0]{\mathbb{Q}}
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\bS}[0]{\mathbb{S}}
\newcommand{\T}[0]{\mathbb{T}}
\newcommand{\X}[0]{\mathfrak{X}}
\newcommand{\Z}[0]{\mathbb{Z}}
\newcommand{\one}[0]{\mathbbm{1}}
%lowercase
\newcommand{\mba}[0]{\mathbf{a}}%idele a
\newcommand{\ma}[0]{\mathfrak{a}}%ideal a
\newcommand{\mb}[0]{\mathfrak{b}}
\newcommand{\mc}[0]{\mathfrak{c}}
\newcommand{\mfd}[0]{\mathfrak d}
\newcommand{\mf}[0]{\mathfrak{f}}
\newcommand{\fg}[0]{\mathfrak{g}}
\newcommand{\vi}[0]{\mathbf{i}}%vector i
\newcommand{\vj}[0]{\mathbf{j}}
\newcommand{\vk}[0]{\mathbf{k}}
\newcommand{\mm}[0]{\mathfrak{m}}%ideal m
\newcommand{\mfp}[0]{\mathfrak{p}}
\newcommand{\mq}[0]{\mathfrak{q}}
\newcommand{\mr}[0]{\mathfrak{r}}
\newcommand{\mv}[0]{\mathbf{v}}
\newcommand{\mx}[0]{\mathbf{x}}%idele x
\newcommand{\my}[0]{\mathbf{y}}
%More sequences of letters
\newcommand{\et}[0]{_{\text{\'et}}}
\newcommand{\Gm}[0]{\mathbb{G}_m}
\newcommand{\Fp}[0]{\mathbb{F}_p}
\newcommand{\fq}[0]{\mathbb{F}_q}
\newcommand{\fpb}[0]{\ol{\mathbb{F}_p}}
\newcommand{\fpt}[0]{\mathbb{F}_p^{\times}}
\newcommand{\fqt}[0]{\mathbb{F}_q^{\times}}
\newcommand{\Kt}[0]{K^{\times}}
\newcommand{\RP}[0]{\mathbb{R}\textup{P}}
\newcommand{\qb}[0]{\ol{\mathbb{Q}}}
\newcommand{\qp}[0]{\mathbb{Q}_p}
\newcommand{\qpb}[0]{\ol{\mathbb{Q}_p}}
\newcommand{\ql}[0]{\mathbb Q_{\ell}}
\newcommand{\sll}[0]{\mathfrak{sl}}
\newcommand{\vl}[0]{V_{\ell}}
\newcommand{\zl}[0]{\mathbb Z_{\ell}}
\newcommand{\zp}[0]{\mathbb Z_{p}}
\newcommand{\zpz}[0]{\mathbb Z/p\mathbb Z}
%Shortcuts for greek letters
\newcommand{\al}[0]{\alpha}
\newcommand{\be}[0]{\beta}
\newcommand{\ga}[0]{\gamma}
\newcommand{\Ga}[0]{\Gamma}
\newcommand{\de}[0]{\delta}
\newcommand{\De}[0]{\Delta}
\newcommand{\ep}[0]{\varepsilon}
\newcommand{\eph}[0]{\frac{\varepsilon}{2}}
\newcommand{\ept}[0]{\frac{\varepsilon}{3}}
\newcommand{\ka}[0]{\kappa}
\newcommand{\la}[0]{\lambda}
\newcommand{\La}[0]{\Lambda}
\newcommand{\ph}[0]{\varphi}
\newcommand{\Ph}[0]{\Phi}
\newcommand{\rh}[0]{\rho}
\newcommand{\te}[0]{\theta}
\newcommand{\Te}[0]{\Theta}
\newcommand{\vte}[0]{\vartheta}
\newcommand{\om}[0]{\omega}
\newcommand{\Om}[0]{\Omega}
\newcommand{\si}[0]{\sigma}
\newcommand{\Si}[0]{\Sigma}
\newcommand{\ze}[0]{\zeta}

%SYMBOLS

%Shortcuts for symbols
\newcommand{\nin}[0]{\not\in}
\newcommand{\opl}[0]{\oplus}
\newcommand{\bigopl}[0]{\bigoplus}
\newcommand{\ot}[0]{\otimes}
\newcommand{\bigot}[0]{\bigotimes}
\newcommand{\sub}[0]{\subset}
\newcommand{\nsub}[0]{\not\subset}
\newcommand{\subeq}[0]{\subseteq}
\newcommand{\supeq}[0]{\supseteq}
\newcommand{\nsubeq}[0]{\not\subseteq}
\newcommand{\nsupeq}[0]{\not\supseteq}
\newcommand{\nequiv}[0]{\not\equiv}
\newcommand{\bs}[0]{\backslash}
\newcommand{\iy}[0]{\infty}
\newcommand{\no}[0]{\trianglelefteq}%normal subgroup
\newcommand{\qeq}[0]{\stackrel?=}
\newcommand{\subsim}[0]{\stackrel{\sub}{\sim}}
\newcommand{\supsim}[0]{\stackrel{\supset}{\sim}}
\newcommand{\na}[0]{\nabla}
\newcommand{\mcv}[0]{*_-}
\newcommand{\dlim}[0]{\varinjlim}
\newcommand{\ilim}[0]{\varprojlim}
\newcommand{\gle}[0]{\begin{array}{c}
\ge\\
\le
\end{array}}
\newcommand{\lge}[0]{\begin{array}{c}
\le\\
\ge
\end{array}}
%\stackrel{-}{*}}%minus convoluion.

%COMMON TIME-SAVERS

%Fractions
\newcommand{\rc}[1]{\frac{1}{#1}}
\newcommand{\prc}[1]{\pa{\rc{#1}}}
\newcommand{\ff}[2]{\left\lfloor\frac{#1}{#2}\right\rfloor}
\newcommand{\cf}[2]{\left\lceil\frac{#1}{#2}\rceil\rfloor}
\newcommand{\fc}[2]{\frac{#1}{#2}}
\newcommand{\sfc}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\pf}[2]{\pa{\frac{#1}{#2}}}%Shortcut for fraction with parentheses
\DeclareRobustCommand{\stl}{\genfrac\{\}{0pt}{}}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}%Partial derivatives
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\pdd}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ddd}[1]{\frac{d}{d #1}}
\newcommand{\af}[2]{\ab{\fc{#1}{#2}}}
\newcommand{\ddt}[2]{\frac{d^2 #1}{d {#2}^2}}
\newcommand{\pdt}[2]{\frac{\partial^2 #1}{\partial {#2}^2}}
\newcommand{\pdxy}[3]{\frac{\partial^2 #1}{\partial {#2}\partial {#3}}}
\newcommand{\pl}[0]{\partial}
\newcommand{\nb}[0]{\nabla}
\newcommand{\onb}[0]{\ol{\nabla}}
\newcommand{\dy}{\,dy}
\newcommand{\dx}{\,dx}

%Arrows
\newcommand{\lar}[0]{\leftarrow}
\newcommand{\ra}[0]{\rightarrow}
\newcommand{\dra}[0]{\dashrightarrow}
\newcommand{\lra}[0]{\leftrightarrow}
\newcommand{\rra}[0]{\twoheadrightarrow}
\newcommand{\hra}[0]{\hookrightarrow}
\newcommand{\tra}[0]{\twoheadrightarrow}
\newcommand{\send}[0]{\mapsto}
\newcommand{\xra}[1]{\xrightarrow{#1}}
\newcommand{\xla}[1]{\xleftarrow{#1}}
\newcommand{\xhra}[1]{\xhookrightarrow{#1}}
\newcommand{\xlra}[1]{\xleftrightarrow{#1}}
\newcommand{\xrc}[0]{\xrightarrow{\cong}}
\renewcommand{\cir}[0]{\circlearrowright}
\newcommand{\cil}[0]{\circlearrowleft}

%Brackets
\newcommand{\ab}[1]{\left| {#1} \right|}
\newcommand{\an}[1]{\left\langle {#1}\right\rangle}
\newcommand{\ba}[1]{\left[ {#1} \right]}
\newcommand{\bc}[1]{\left\{ {#1} \right\}}
\newcommand{\bra}[1]{\langle{#1}|}
\newcommand{\braa}[1]{\langle\langle{#1}|}
\newcommand{\ce}[1]{\left\lceil {#1}\right\rceil}
\newcommand{\fl}[1]{\left\lfloor {#1}\right\rfloor}
\newcommand{\ro}[1]{\left\lfloor {#1}\right\rceil}
\newcommand{\ket}[1]{|{#1}\rangle}
\newcommand{\kett}[1]{|{#1}\rangle\rangle}
\newcommand{\bk}[2]{\langle{#1}|{#2}\rangle}
\newcommand{\bok}[3]{\langle{#1}|{#2}|{#3}\rangle}
\newcommand{\braak}[2]{\langle\langle{#1}|{#2}\rangle\rangle}
\newcommand{\kbb}[1]{|{#1}\rangle\langle{#1}|}
\newcommand{\kb}[2]{|{#1}\rangle\langle{#2}|}
\newcommand{\kettb}[2]{|{#1}\rangle\rangle\langle\langle{#2}|}
\newcommand{\pa}[1]{\left( {#1} \right)}
\newcommand{\pat}[1]{\left( \text{#1} \right)}
\newcommand{\ve}[1]{\left\Vert {#1}\right\Vert}
\newcommand{\nv}[1]{\frac{#1}{\left\Vert {#1}\right\Vert}}
\newcommand{\nvl}[2]{\frac{#1}{\left\Vert {#1}\right\Vert_{#2}}}
\newcommand{\vvt}[1]{{#1}{#1}^\top}
\newcommand{\pvvt}[1]{\pa{#1}\pa{#1}^\top}
\newcommand{\vtv}[1]{{#1}^\top{#1}}
\newcommand{\pvtv}[1]{\pa{#1}^\top\pa{#1}}
\newcommand{\rb}[1]{\left.{#1}\right|}
%\newcommand{\nl}[1]{\left\Vert #1 \right\Vert_{L^1}}
\newcommand{\ad}[0]{|\cdot|}
\newcommand{\ved}[0]{\ve{\cdot}}
\renewcommand{\set}[2]{\left\{{#1}:{#2}\right\}}
\newcommand{\sett}[2]{\left\{\left.{#1}\right|{#2}\right\}}

%under and overlines, etc.
\newcommand{\ch}[1]{\check{#1}}
\newcommand{\dch}[1]{\check{\check{#1}}}
\newcommand{\olra}[1]{\overleftrightarrow{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\ub}[2]{\underbrace{#1}_{#2}}
\newcommand{\ora}[1]{\overrightarrow{#1}}
\newcommand{\ura}[1]{\underrightarrow{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}

%other
\newcommand{\fp}[1]{^{\underline{#1}}}%Falling power
\newcommand{\rp}[1]{^{\overline{#1}}}
\newcommand{\pp}[1]{^{(#1)}}
\newcommand{\sh}[0]{^{\sharp}}
\newcommand{\ri}[0]{\ddagger}%replace this with rosati involution
\newcommand{\bit}[0]{\{0,1\}}

%TEXT
\newcommand{\btih}[1]{\text{ by the induction hypothesis{#1}}}
\newcommand{\bwoc}[0]{by way of contradiction}
\newcommand{\by}[1]{\text{by~(\ref{#1})}}
\newcommand{\idk}[0]{{\color{red}I don't know.} }
\newcommand{\ore}[0]{\text{ or }}
\newcommand{\wog}[0]{ without loss of generality }
\newcommand{\Wog}[0]{ Without loss of generality }
\newcommand{\step}[1]{\noindent{\underline{Step {#1}:}}}
\newcommand{\prt}[1]{\noindent{\underline{Part {#1}:}}}
\newcommand{\tfae}[0]{ the following are equivalent}
\newcommand{\fabfm}[0]{for all but finitely many }

%FUNCTIONS
%Functions, etc.
\newcommand{\Abs}{(\text{Ab}/S)}
\newcommand{\abk}{(\text{Ab}/k)}
\newcommand{\abc}{(\text{Ab}/\C)}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\amax}{\operatorname{argmax}}
\newcommand{\amin}{\operatorname{argmin}}
\newcommand{\Ass}{\operatorname{Ass}}
\newcommand{\Art}{\operatorname{Art}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\avg}{\operatorname{avg}}
\newcommand{\bias}[0]{\operatorname{bias}}
\newcommand{\Bin}{\operatorname{Bin}}
\newcommand{\Binom}{\operatorname{Binom}}
\newcommand{\Bl}[0]{\operatorname{Bl}}
\newcommand{\Br}{\operatorname{Br}}
\newcommand{\chr}{\operatorname{char}}
\newcommand{\cis}{\operatorname{cis}}
\newcommand{\cl}{\operatorname{Cl}}
%\newcommand{\Cl}{C}%changed notation%this is confusing
\newcommand{\Cl}{\operatorname{Cl}}
\newcommand{\Coh}{\operatorname{Coh}}
\newcommand{\Coinf}[0]{\operatorname{Coinf}}
\newcommand{\Coind}[0]{\operatorname{Coind}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Comp}{\operatorname{Comp}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\oconv}{\ol{\conv}}
\newcommand{\Cor}{\operatorname{Cor}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\cro}{\operatorname{cr}}
\newcommand{\degs}[0]{\deg_{\text{s}}}%separable degree
\newcommand{\Dec}{\operatorname{Dec}}
\newcommand{\depth}{\operatorname{depth}}
\newcommand{\Der}{\operatorname{Der}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\diam}{\operatorname{diam}}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\Dir}{\operatorname{Dir}}
\newcommand{\Div}{\operatorname{Div}}
\newcommand{\Disc}{\operatorname{Disc}}%discrepancy
\newcommand{\disc}{\operatorname{disc}}%discriminant
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\Ell}{\mathcal{E}{\rm{ll}}}
\newcommand{\Enc}{\operatorname{Enc}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ent}{\operatorname{Ent}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\Exp}{\operatorname{Exp}}
\newcommand{\err}{\operatorname{err}}
\newcommand{\ess}{\operatorname{ess}}
\newcommand{\ext}{\operatorname{ext}}
\newcommand{\pfcg}{(p\text{-FCGp}/k)}
\newcommand{\fcg}{(\text{FCGp}/k)}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\FS}{\operatorname{FS}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Gap}{\operatorname{Gap}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\gps}{(\text{Gp}/S)}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\Het}{H_{\text{\'et}}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Homeo}{\operatorname{Homeo}}
\newcommand{\chom}[0]{\mathscr{H}om}
\newcommand{\Homc}{\operatorname{Hom}_{\text{cont}}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\im}[0]{\text{im}}
\newcommand{\imp}[0]{\im^{\text{pre}}}
\newcommand{\Ind}[0]{\operatorname{Ind}}
\newcommand{\Inf}[0]{\operatorname{Inf}}
\newcommand{\inv}[0]{\operatorname{inv}}
\newcommand{\Isoc}[0]{\operatorname{Isoc}}
\newcommand{\Isog}[0]{\operatorname{Isog}}
\newcommand{\Isom}[0]{\operatorname{Isom}}
\newcommand{\KL}[0]{\operatorname{KL}}
\newcommand{\Jac}[0]{\operatorname{Jac}}
\newcommand{\li}[0]{\operatorname{li}}
\newcommand{\Li}[0]{\operatorname{li}}
\newcommand{\Lie}[0]{\operatorname{Lie}}
\newcommand{\Line}[0]{\operatorname{Line}}
\newcommand{\Lip}[0]{\operatorname{Lip}}
\newcommand{\lcm}[0]{\operatorname{lcm}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Dmod}{\Mod_{W[F,V]}^{\text{fl}}}
\newcommand{\nil}[0]{\operatorname{nil}}
\newcommand{\nm}{\operatorname{Nm}}
\newcommand{\NS}{\operatorname{NS}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\PDer}{\operatorname{PDer}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Pico}{\operatorname{Pic}^{\circ}}
\newcommand{\Pois}{\operatorname{Pois}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\polylog}{\operatorname{polylog}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\Per}{\operatorname{Per}}
\newcommand{\perm}{\operatorname{perm}}
\newcommand{\PrePer}{\operatorname{PrePer}}
\newcommand{\Prob}{\operatorname{Prob}}
\newcommand{\Proj}{\operatorname{Proj}}
\newcommand{\Prj}[0]{\textbf{Proj}}
\newcommand{\QCoh}{\operatorname{QCoh}}
\newcommand{\Rad}{\operatorname{Rad}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\red}{\operatorname{red}}
\newcommand{\Reg}{\operatorname{Reg}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\Ric}{\operatorname{Ric}} %Ricci curvature
\newcommand{\rot}{\operatorname{rot}}
\newcommand{\Scal}{\operatorname{Scal}} %Ricci curvature
\newcommand{\schs}{(\text{Sch}/S)}
\newcommand{\schk}{(\text{Sch}/k)}
\newcommand{\se}{\text{se}}
\newcommand{\srank}{\text{srank}}
\newcommand{\hse}{\wh{\text{se}}}
\newcommand{\Sel}{\operatorname{Sel}}
\newcommand{\sens}{\operatorname{sens}}
\newcommand{\Set}{(\text{Set})}
\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spec}{\operatorname{Spec}}
\newcommand{\Specf}[2]{\Spec\pa{\frac{k[{#1}]}{#2}}}
\newcommand{\rspec}{\ul{\operatorname{Spec}}}
\newcommand{\Spl}{\operatorname{Spl}}
\newcommand{\spp}{\operatorname{sp}}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Supp}{\operatorname{Supp}}
\newcommand{\ssupp}{\operatorname{sing}\operatorname{supp}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Th}{\operatorname{Th}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\tor}{\operatorname{tor}}
\newcommand{\Tr}[0]{\operatorname{Tr}}
\newcommand{\tr}[0]{\operatorname{tr}}
\newcommand{\val}[0]{\text{val}}
\newcommand{\Var}[0]{\operatorname{Var}}
\newcommand{\var}[0]{\text{var}}
\newcommand{\vcong}{\operatorname{vcong}}
\newcommand{\Vol}[0]{\text{Vol}}
\newcommand{\vol}[0]{\text{vol}}
\providecommand{\cal}[1]{\mathcal{#1}}
\renewcommand{\cal}[1]{\mathcal{#1}}
\providecommand{\bb}[1]{\mathbb{#1}}
\renewcommand{\bb}[1]{\mathbb{#1}}

%Text super/subscripts
\newcommand{\abe}[0]{^{\text{ab}}}
\newcommand{\gal}[0]{^{\text{gal}}}%galois closure
\newcommand{\op}{^{\text{op}}}
\newcommand{\pre}[0]{^{\text{pre}}}
\newcommand{\rd}[0]{_{\text{red}}}
\newcommand{\sep}[0]{^{\text{sep}}}
\newcommand{\tp}{^{\text{top}}}
\newcommand{\tors}{_{\text{tors}}}
\newcommand{\ur}[0]{^{\text{ur}}}
\newcommand{\urt}[0]{^{\text{ur}\times}}

%COMMUTATIVE DIAGRAMS

%Commutative diagram shortcuts
\newcommand{\commsq}[8]{\xymatrix{#1\ar[r]^-{#6}\ar[d]_{#5} &#2\ar[d]^{#7} \\ #3 \ar[r]^-{#8} & #4}}
%Makes a diagram like this
%1->2
%|    |
%3->4
%Arguments 5, 6, 7, 8 on arrows
%  6
%5  7
%  8
\newcommand{\pull}[9]{
#1\ar@/_/[ddr]_{#2} \ar@{.>}[rd]^{#3} \ar@/^/[rrd]^{#4} & &\\
& #5\ar[r]^{#6}\ar[d]^{#8} &#7\ar[d]^{#9} \\}
\newcommand{\back}[3]{& #1 \ar[r]^{#2} & #3}
%Syntax:\pull 123456789 \back ABC
%1=upper left-hand corner
%2,3,4=arrows from upper LH corner, going down, diagonal, right
%5,6,7=top row (6 on arrow)
%8,9=middle rows (on arrows)
%A,B,C=bottom row
%composition
\newcommand{\cmp}[9]{
\xymatrix{
#1 \ar[r]^{#4}{#5} \ar@/_2pc/[rr]^{#8}_{#9} & #2 \ar[r]^{#6}_{#7} & #3
}
}
\newcommand{\ctr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\ar[ld]_{#8}^{#9}\\
& #3 &
}
}
\newcommand{\ctrr}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5} && #2\\
& #3 \ar[lu]_{#6}^{#7}\ar[ru]_{#8}^{#9}&
}
}

\newcommand{\ctri}[9]{
\xymatrix{
#1 \ar[rr]^{#4}_{#5}\ar[rd]^{#6}_{#7} && #2\\
& #3 \ar[ru]^{#8}_{#9}&
}
}
\newcommand{\rcommsq}[8]{\xymatrix{#1 &#2\ar[l]_-{#6} \\ #3 \ar[u]^{#5} & #4 \ar[u]_{#7}\ar[l]_-{#8}}}


%Arrow shortcuts
\newcommand{\ha}[1]{\ar@{^(->}[#1]}
\newcommand{\ls}[1]{\ar@{-}[#1]}
\newcommand{\sj}[1]{\ar@{->>}[#1]}
\newcommand{\aq}[1]{\ar@{=}[#1]}
\newcommand{\acir}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowright}}}
\newcommand{\acil}[1]{\ar@{}[#1]|-{\textstyle{\circlearrowleft}}}
\newcommand{\ard}[1]{\ar@{.>}[#1]}
\newcommand{\mt}[1]{\ar@{|->}[#1]}
\newcommand{\inm}[1]{\ar@{}[#1]|-{\in}}
\newcommand{\inr}{\ar@{}[d]|-{\rotatebox[origin=c]{-90}{$\in$}}}
\newcommand{\inl}{\ar@{}[u]|-{\rotatebox[origin=c]{90}{$\in$}}}

%Other
%\newcommand{\set}[2]{\left.\left\{{#1}\right|{#2}\right\}}
%\newcommand{\sett}[2]{\left\{{#1}\left|{#2}\right\}\right.}

%SUMS, ETC.
\newcommand{\sumr}[2]{\sum_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%sum with 2 rows
\newcommand{\prr}[2]{\prod_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\maxr}[2]{\max_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\minr}[2]{\min_{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}}%product with 2 rows
\newcommand{\trow}[2]{\scriptsize \begin{array}{c}{#1}\\{#2}\end{array}}
\newcommand{\seqo}[3]{\{#3\}_{#1=1}^{#2}}
\newcommand{\seqos}[3]{\{#3_#1\}_{#1=1}^{#2}}
\newcommand{\seqz}[3]{\{#3\}_{#1=0}^{#2}}
\newcommand{\seqzs}[3]{\{#3_#1\}_{#1=0}^{#2}}
\newcommand{\su}[0]{\sum_{n=0}^{\iy}}
\newcommand{\suo}[0]{\sum_{n=1}^{\iy}}
\newcommand{\sumo}[2]{\sum_{#1=1}^{#2}}
\newcommand{\sumz}[2]{\sum_{#1=0}^{#2}}
\newcommand{\prodo}[2]{\prod_{#1=1}^{#2}}
\newcommand{\prodz}[2]{\prod_{#1=0}^{#2}}
\newcommand{\oplo}[2]{\bigopl_{#1=1}^{#2}}
\newcommand{\cupo}[2]{\bigcup_{#1=1}^{#2}}
\newcommand{\capo}[2]{\bigcap_{#1=1}^{#2}}
\newcommand{\iiy}[0]{\int_0^{\infty}}
\newcommand{\iny}[0]{\int_{-\infty}^{\infty}}
\newcommand{\iiiy}[0]{\int_{-\infty}^{\infty}}%DEPRECATED
\newcommand{\sui}[0]{\sum_{i=1}^{n}}
\newcommand{\suiy}[0]{\sum_{i=1}^{\iy}}
\newcommand{\cui}[0]{\bigcup_{i=1}^n}
\newcommand{\suj}[0]{\sum_{j=1}^{n}}
\newcommand{\suij}[0]{\sum_{i,j}}
\newcommand{\limn}[0]{\lim_{n\to \infty}}

%MATRICES

%Matrices
\newcommand{\scoltwo}[2]{
\left(\begin{smallmatrix}
{#1}\\
{#2}
\end{smallmatrix}\right)}
\newcommand{\coltwo}[2]{
\begin{pmatrix}
{#1}\\
{#2}
\end{pmatrix}}
\newcommand{\colthree}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\colfour}[4]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}\\
{#4}
\end{pmatrix}
}
\newcommand{\cth}[3]{
\begin{pmatrix}
{#1}\\
{#2}\\
{#3}
\end{pmatrix}
}
\newcommand{\detm}[4]{
\ab{
\begin{matrix}
{#1}&{#2}\\
{#3}&{#4}
\end{matrix}
}}
\newcommand{\sdetm}[4]{
\ab{
\begin{smallmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}
}}
\newcommand{\matt}[4]{
\begin{pmatrix}
{#1}&{#2}\\
{#3}&{#4}
\end{pmatrix}
}
\newcommand{\smatt}[4]{
\left(\begin{smallmatrix} 
{#1}&{#2}\\
{#3}&{#4}
\end{smallmatrix}\right)
}
\newcommand{\mattn}[9]{
\begin{pmatrix}
{#1}&{#2}&{#3}\\
{#4}&{#5}&{#6}\\
{#7}&{#8}&{#9}
\end{pmatrix}
}

\newcommand{\bt}[2]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}
\end{matrix}
\right\}}
\newcommand{\bth}[3]{
\left\{\begin{matrix}
\text{#1}\\
\text{#2}\\
\text{#3}
\end{matrix}
\right\}}

\newcommand{\tcase}[4]{
\begin{cases}
#1 & #2\\
#3 & #4
\end{cases}}
\newcommand{\txcase}[4]{
\begin{cases}
#1 & \text{#2}\\
#3 & \text{#4}
\end{cases}}

\newcommand{\ifoth}[3]{
\begin{cases}
#1 & \text{if }#2\\
#3 & \text{otherwise}
\end{cases}}

%EQUATIONS
\newcommand{\beq}[1]{\begin{equation}\llabel{#1}}
\newcommand{\eeq}[0]{\end{equation}}
\newcommand{\bal}[0]{\begin{align*}}
\newcommand{\eal}[0]{\end{align*}}%this doesn't work; i don't know why
\newcommand{\ban}[0]{\begin{align}}
\newcommand{\ean}[0]{\end{align}}
\newcommand{\ig}[2]{\begin{center}\includegraphics[scale=#2]{#1}\end{center}}
\newcommand{\ign}[2]{\includegraphics[scale=#2]{#1}}

%COURSE-SPECIFIC

%measure theory, analysis
\newcommand{\am}[0]{(a.e., $\mu$)}
\newcommand{\ftla}[1]{\int e^{i\lambda\cdot x}{#1}\,d\lambda}
\newcommand{\lime}[0]{\lim_{\varepsilon\to 0}}

%number theory
\newcommand{\modt}[1]{\,(\text{mod}^{\times}\, {#1})}
\newcommand{\tl}[0]{T_{\ell}}
 %multiplicative subgroup
\newcommand{\zmod}[1]{\Z/{#1}\Z}
\newcommand{\md}[1]{\,(\text{mod }#1)}
\newcommand{\ks}[1]{K(\sqrt{#1})}
\newcommand{\ksq}[1]{K(\sqrt{#1})/K}
\newcommand{\nksq}[1]{\nm_{K(\sqrt{#1})/K}(K(\sqrt{#1})^{\times})}
\newcommand{\mpp}[0]{\mP/\mfp}

%manifolds
\newcommand{\cvd}[0]{\frac{D}{\partial t}}
\newcommand{\cvs}[0]{\frac{D}{\partial s}}
\newcommand{\np}[1]{\nabla_{\pd{}{#1}}}

%algebraic geometry
\newcommand{\av}[0]{A^{\vee}}


%arithmetic combinatorics
\newcommand{\Deq}[1]{\Delta^{\times}_{#1}}

%modular forms
\newcommand{\GLAi}[0]{\text{GL}_2(\mathbb A)_{\infty}}

%noise sensitivity part iii essay
\newcommand{\Dict}[0]{\operatorname{\mathsf{Dict}}}
\newcommand{\Maj}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\MAJ}[0]{\operatorname{\mathsf{Maj}}}
\newcommand{\Parity}[0]{\operatorname{\mathsf{Parity}}}
\newcommand{\Tribes}[0]{\operatorname{\mathsf{Tribes}}}
\newcommand{\Ns}[0]{\operatorname{NS}}
\newcommand{\DT}[0]{\operatorname{\mathsf{DT}}}
\newcommand{\DNF}[0]{\operatorname{\mathsf{DNF}}}
\newcommand{\CNF}[0]{\operatorname{\mathsf{CNF}}}
\newcommand{\Circuit}[0]{\operatorname{\mathsf{Circuit}}}
\newcommand{\Ac}[0]{\mathsf{AC}}
\newcommand{\EB}[0]{\text{EB}}
%comp complexity
%complexity theory
\newcommand{\ACC}[0]{\operatorname{\mathsf{ACC}}}
\newcommand{\BPP}[0]{\mathsf{BPP}}
\newcommand{\BPTIME}[0]{\operatorname{\mathsf{BPTIME}}}
\newcommand{\CLIQUE}[0]{\operatorname{\mathsf{CLIQUE}}}
\newcommand{\EXP}[0]{\mathsf{EXP}}
\newcommand{\NEXP}[0]{\mathsf{NEXP}}
\newcommand{\NC}[0]{\operatorname{\mathsf{NC}}}
\newcommand{\NP}[0]{\operatorname{\mathsf{NP}}}
\newcommand{\NTIME}[0]{\operatorname{\mathsf{NTIME}}}
\newcommand{\msP}[0]{\operatorname{\mathsf{P}}}
\newcommand{\PCP}[0]{\operatorname{\mathsf{PCP}}}
\newcommand{\SAT}[0]{\mathsf{SAT}}
\newcommand{\SUBEXP}[0]{\mathsf{SUBEXP}}
\newcommand{\TIME}[0]{\operatorname{\mathsf{TIME}}}
\newcommand{\zz}{\textcircled{Z}}
%statistics
\newcommand{\hten}[0]{\widehat{\theta_n}}

%EDITING HELP
%blu: key idea or concept. red: unresolved issue/question. 
\newcommand{\blu}[1]{{\color{blue}#1}}
\newcommand{\grn}[1]{{\color{green}#1}}
\newcommand{\redd}[1]{{\color{red}#1}}
\newcommand{\pur}[1]{{\color{purple}#1}}
\newcommand{\oge}[1]{{\color{orange}#1}}
\newcommand{\concept}[1]{#1}
\newcommand{\fixme}[1]{{\color{red}#1}}
\newcommand{\hlnote}[1]{{\color{red}HL: #1}}
\newcommand{\cary}[1]{{\color{purple}#1}}%deprecated
%short for commentary
\newcommand{\llabel}[1]{\label{#1}\text{\fixme{\tiny#1}}}
\newcommand{\nref}[1]{\ref{#1}}
%%%%%%%%%%%
%Use the above when working on the document, so labels will be displayed by their theorems, and you can write reminders to yourself. Switch to the below commands when publishing.
%%%%%%%%%%%
%\newcommand{\fixme}[1]{}
%\newcommand{\concept}[1]{{\color{blue}#1}}
%\newcommand{\llabel}[1]{\label{#1}}
%%%%%%%%%%%

\newcommand{\itag}[1]{\index{#1}[\##1]}
\newcommand{\ilbl}[1]{[#1]\index{#1}}
\newcommand{\iadd}[1]{\index{#1} #1}
\newcommand{\arxiv}[1]{\url{http://www.arxiv.org/abs/#1}}

%markup
\newcommand{\ivocab}[1]{\index{#1}\textbf{#1}}
\newcommand{\vocab}[1]{\emph{#1}} %also index automatically.
\newcommand{\summq}[1]{\textbf{Summary Question: }#1}
\newcommand{\keypt}[1]{{\it #1}}
\newcommand{\subprob}[1]{\noindent\textbf{#1}\\}
\newcommand{\qatable}[1]{\begin{center}
    \begin{longtable}{ | p{5.5cm} | p{10cm} |}
#1
\end{longtable}
\end{center}}

%Page breaks in equations
\allowdisplaybreaks[2]

%SHA
\DeclareFontFamily{U}{wncy}{}
    \DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
    \DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
    \DeclareMathSymbol{\Sh}{\mathord}{mcy}{"58} 

==> main-alt.tex <==
% \documentclass[anon,12pt]{alt2021} % Anonymized submission
% % \documentclass[12pt]{alt2021} % Include author names

% % The following packages will be automatically loaded:
% % amsmath, amssymb, natbib, graphicx, url, algorithm2e

% \title[Efficient sampling from the Bingham distribution]{Efficient sampling from the Bingham distribution}
% \usepackage{times}



% %\usepackage{times}
% \usepackage{algorithm,algorithmicx,algpseudocode}
% %%main packages
% %\usepackage{amsmath}
% %\usepackage{amssymb}
% %\usepackage{amsthm}
% \usepackage{array}
% \usepackage{bbm}
% %\usepackage{asymptote}
% \usepackage{cancel}
% \usepackage{color}
% \usepackage{cmap}
% \usepackage{enumerate}
% \usepackage{enumitem}%resume lists
% %\usepackage{makeidx}
% %\usepackage{marvosym}%doesn't work
% \usepackage{mathtools}
% \usepackage{mathrsfs}
% \usepackage{hyperref}
% %\usepackage{sidecap}
% \usepackage{stackrel}
% \usepackage{stmaryrd}%\mapsfrom
% \usepackage{url}
% \usepackage{verbatim}
% \usepackage{wasysym}
% \usepackage{wrapfig}
% \usepackage{yhmath}
% %\usepackage{yhmath}%arcs
% \usepackage[all,cmtip]{xy}%Commutative diagrams
% %\usepackage[usenames,dvipsnames]{xcolor}%tikz loads xcolor

% \newcommand{\sech}[0]{\operatorname{sech}}

% %load hyperref last
% \usepackage{hyperref}

% %https://tex.stackexchange.com/questions/51286/recalling-a-theorem
% \usepackage{thmtools}
% \usepackage{thm-restate}
% \usepackage{cleveref}

% %%%%%%%%%%%%%%%%%%%%%%%%%
% %\usepackage[backend=biber,style=alphabetic]{biblatex}
% \input{theorems_std.tex}
% \input{macros-alt.tex}
% \renewcommand{\llabel}[1]{\label{#1}}
% \newcommand{\jl}[1]{\textcolor{magenta}{[JL: #1]}}
% \newcommand{\andr}[1]{\textcolor{red}{[andrej: #1]}}



% % Use \Name{Author Name} to specify the name.
% % If the surname contains spaces, enclose the surname
% % in braces, e.g. \Name{John {Smith Jones}} similarly
% % if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% % If the first letter in the forenames is a diacritic
% % enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% % Two authors with the same address
% % \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
% %  \Name{Author Name2} \Email{xyz@sample.com}\\
% %  \addr Address}

% % Three or more authors with the same address:
% % \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
% %  \Name{Author Name2} \Email{an2@sample.com}\\
% %  \Name{Author Name3} \Email{an3@sample.com}\\
% %  \addr Address}

% % Authors with different addresses:
% \altauthor{%
%  \Name{Rong Ge} \Email{}\\
%  \Name{Holden Lee} \Email{}\\
%  \Name{Jianfeng Lu} \Email{}\\ 
%  \addr Duke University
%  \AND
%  \Name{Andrej Risteski} \Email{}\\
%  \addr Carnegie Mellon University
% }

% \begin{document}

% \maketitle

% \input{intro}
% \input{polynomial}
% \input{conclusion}

% % Acknowledgments---Will not appear in anonymized version
% %\acks{We thank a bunch of people.}

% \bibliography{bib}

% \appendix

% \input{moment}

% \end{document}


==> theorems_with_boxes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Theorem styles
\newtheoremstyle{norm}
{12pt}
{12pt}
{}
{}
{\bf}
{:}
{.5em}
{}

\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm*}{Theorem}
\newtheorem{clm}[thm]{Claim}
\newtheorem*{clm*}{Claim}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem*{conj*}{Conjecture}
%\newtheorem{cons}{Construction}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem*{lem*}{Lemma}

\theoremstyle{norm}
\newtheorem{prb}[thm]{Problem}%[section]
\newtheorem*{prb*}{Problem}

\newtheorem{alg}[thm]{Algorithm}
\newtheorem{assm}[thm]{Assumption}
\newtheorem{ax}[thm]{Axiom}
\newtheorem*{ax*}{Axiom}
\newtheorem{df}[thm]{Definition}
\newtheorem*{df*}{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem*{ex*}{Example}
\newtheorem{exr}[thm]{Exercise}
\newtheorem{expl}[thm]{Exploration}%prb
\newtheorem{fct}[thm]{Fact}
\newtheorem{mdl}[thm]{Model}
\newtheorem{pos}[thm]{Postulate}
\newtheorem*{pos*}{Postulate}
%\newtheorem{sprb}{Problem}%numbering for solutions
\newtheorem{pr}[thm]{Proposition}
\newtheorem*{pr*}{Proposition}
\newtheorem{qu}[thm]{Question}
\newtheorem*{qu*}{Question}
\newtheorem{rem}[thm]{Remark}
\newtheorem*{rem*}{Remark}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%DEFINING BOX COMMANDS
\newcommand{\prbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [prbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}
}
\newcommand{\prbbox}[1]{\prbox{\begin{prb}#1\end{prb}}}
\newcommand{\expbox}[1]{\prbox{\begin{expl}#1\end{expl}}}
\newcommand{\sprbbox}[1]{\prbox{\begin{sprb}#1\end{sprb}}}

\newcommand{\thbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [thbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
%6.68

\newcommand{\thmbox}[1]{\thbox{\begin{thm}#1\end{thm}}}
\newcommand{\dfbox}[1]{\thbox{\begin{df*}#1\end{df*}}}

\newcommand{\grbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [cpbox] (box){
\begin{minipage}[l]{6in}
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
\newcommand{\cpbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [cpbox] (box){
\begin{minipage}[c]{.2in}
%\hspace{-.2in}
%\dbend
\includegraphics[scale=0.35]{\filepath/key}
\end{minipage}
\begin{minipage}[t]{6in}%6.25
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}


\newcommand{\wrbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [wrbox] (box){
\begin{minipage}[c]{.2in}
%\hspace{-.2in}
%\dbend
{\Huge \bf !}
\end{minipage}
\begin{minipage}[t]{6in}%6.25
#1
\end{minipage}
};
\end{tikzpicture}\\%
}}
\newcommand{\hintbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [hnbox] (box){
\begin{minipage}[l]{6in}
\textbf{Hint:} {#1}
\end{minipage}
};
\end{tikzpicture}\\%
}
}
%white box
\newcommand{\whbox}[1]{{
\noindent
\centering
\begin{tikzpicture}
\node [hnbox] (box){
\begin{minipage}[l]{6in}
{#1}
\end{minipage}
};
\end{tikzpicture}\\%
}
}
%6.68
%END DEFINING BOX COMMANDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Box commands
%\thbox{...} makes a theorem box
%\thmbox{...} makes a theorem box labeled "Theorem"
%\prbox{...} makes a problem box
%\prbbox{...} makes a problem box labeled "Problem"
%\cpbox{...} makes a concept box labeled "Concept"
%\wrbox{...} makes a warning box.
%\dfbox{...} makes a definition box (same as problem box) labeled "> Definition"
%\sprbbox{...} makes a problem box labeled "Problem" (use this when you're making a copy of a previous problem box to put the solution afterwards; it has a numbering system separate from problems).

 
% for testing purposes only
\usepackage[english]{babel} 
\usepackage{blindtext} 
%%%%%%%%
%begin doc
%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%DEFINING THE BOXES.
% Problem box (simple box, blue)
\tikzstyle{prbox} = [draw=black, fill=blue!20, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
% Theorem box (double border, gray)
\tikzstyle{thbox} = [draw=black,double, fill=blue!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
%\tikzstyle{fancytitle} =[fill=red, text=white]
% Concept box (shadowed, light green)
\tikzstyle{cpbox} = [drop shadow={
    shadow scale=1}, draw=black, fill=green!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
\tikzstyle{wrbox} = [drop shadow={
    shadow scale=1}, draw=black, fill=yellow!10, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
\tikzstyle{hnbox} = [draw=black, fill=white, very thick,
    rectangle, inner sep=10pt, inner ysep=10pt]
%END DEFINING BOXES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

